The University of Michigan Centimeter-Band All Stokes Blazar Monitoring Program: Single-Dish Polarimetry as a Probe of Parsec-Scale Magnetic Fields

The University of Michigan 26-m paraboloid was dedicated to obtaining linear polarization and total flux density observations of blazars from the mid-1960s until June 2012 providing an unprecedented record tracking centimeter-band variability over decades at 14.5, 8.0, and 4.8 GHz for both targeted objects and members of flux-limited samples. In the mid-1970s through the mid-1980s, and during the last decade of the program, observations were additionally obtained of circular polarization for a small sample of radio-bright (S>5Jy), active sources. Key program results include evidence supporting class-dependent differences in the magnetic field geometry of BL Lac and QSO jets, identification of linear polarization changes temporally associated with flux outbursts supporting a shock-in-jet scenario, and determination of the spectral evolution of the Stokes V amplitude and polarity for testing proposed models. Recent radiative transfer modeling during large flares supports a jet scenario with a kinetically-dominated, relativistic flow at parsec scales with embedded turbulent magnetic fields and dynamically-weak ordered components which may be helical; the circular polarization observations are consistent with linear-to-circular mode conversion within this turbulent jet environment.

==> unicode.tex <==

\DeclareUnicodeCharacter{1E45}{\.{n}}
\DeclareUnicodeCharacter{1E41}{\.{m}}
\DeclareUnicodeCharacter{2003}{\quad}
\DeclareUnicodeCharacter{0177}{\^{y}}
\DeclareUnicodeCharacter{101}{\={a}}
\DeclareUnicodeCharacter{2009}{\thinspace}
\DeclareUnicodeCharacter{2002}{\enspace{}}
\DeclareUnicodeCharacter{2005}{\thinspace}
\DeclareUnicodeCharacter{0263}{\textipa{G}}
\DeclareUnicodeCharacter{117}{\.{e}}
\DeclareUnicodeCharacter{A0}{~}
\DeclareUnicodeCharacter{2460}{\textcircled{\scriptsize{1}}}
\DeclareUnicodeCharacter{2461}{\textcircled{\scriptsize{2}}}
\DeclareUnicodeCharacter{2462}{\textcircled{\scriptsize{3}}}
\DeclareUnicodeCharacter{2463}{\textcircled{\scriptsize{4}}}
\DeclareUnicodeCharacter{2464}{\textcircled{\scriptsize{5}}}
\DeclareUnicodeCharacter{2465}{\textcircled{\scriptsize{6}}}
\DeclareUnicodeCharacter{2466}{\textcircled{\scriptsize{7}}}
\DeclareUnicodeCharacter{2467}{\textcircled{\scriptsize{8}}}
\DeclareUnicodeCharacter{2468}{\textcircled{\scriptsize{9}}}
\DeclareUnicodeCharacter{02C2}{<}
\DeclareUnicodeCharacter{2033}{''}
\DeclareUnicodeCharacter{0229}{\c{e}}
\DeclareUnicodeCharacter{0218}{\cb{S}}
\DeclareUnicodeCharacter{0219}{\cb{s}}
\DeclareUnicodeCharacter{021B}{\cb{t}}
